Measurement of the Two-Neutrino Double Beta Decay Half-life of $^{130}$Te with the CUORE-0 Experiment

We report on the measurement of the two-neutrino double beta decay half-life of $^{130}$Te with the CUORE-0 detector. From an exposure of 33.4 kg$\cdot$y of TeO$_2$, the half-life is determined to be $T_{1/2}^{2\nu}$ = [8.2 $\pm$ 0.2 (stat.) $\pm$ 0.6 (syst.)] $\times$ 10$^{20}$y. This result is obtained after a detailed reconstruction of the sources responsible for the CUORE-0 counting rate, with a specific study of those contributing to the $^{130}$Te neutrinoless double beta decay region of interest.

==> FitList.tex <==
\def\ums{$\mu$m}


\begin{table*}
\begin{center}
\begin{small}
\caption{List of the sources and priors used to fit the \qz~ background data. If not differently specified, \ths, \us and $^{210}$Pb refer to the whole decay chains in secular equilibrium.}	
\begin{tabular}{lll|lll}
\hline
\textbf{Source}	&	\textbf{Prior (Bq/kg)}	& 	\textbf{Posterior (Bq/kg)}	&	\textbf{Source}	&	\textbf{Prior (Bq/kg)}	& 	\textbf{Posterior (Bq/kg)}	
\\
	
\hline
\textbf{Crystal bulk}	&	 					&		&	\textbf{Crystal surfaces}	&	&	\\
\hline
$^{130}$Te-\bbdn		&						&					&	\ths(only)\,--\,0.01\,\ums		&	 &	\\
$^{210}$Po				& 	$(2.4\pm0.1)\times10^{-6}$	& 	$(2.4\pm0.1)\times10^{-6}$	&	$^{228}$Ra-$^{208}$Pb\,--\,0.01\,\ums					& 	$(2.4\pm0.1)\times10^{-6}$	 & 	$(2.4\pm0.1)\times10^{-6}$\\
$^{210}$Pb				&						& &	\us-$^{230}$Th\,--\,0.01\,\ums		&	 &	\\
\ths(only)				&						& &	$^{230}$Th (only)\,--\,0.01\,\ums		&	 &	\\
$^{228}$Ra-$^{208}$Pb	&						& &	$^{226}$Ra-$^{210}$Pb\,--\,0.01\,\ums		&	 &	\\
\us-$^{230}$Th			&						& &	$^{210}$Pb\,--\,0.001\,\ums			&	 &	\\
$^{230}$Th(only)		&						& &	$^{210}$Pb\,--\,1\,\ums				&	 &	\\
$^{226}$Ra-$^{210}$Pb	&						& &	$^{210}$Pb\,--\,10\,\ums				&	 &	\\
\cosn 					&	$<3\times10^{-7}$	& &	\ths\,--\,10\,\ums 			&	 &	\\
$^{40}$K				&	$<1\times10^{-3}$	& &	\us\,--\,10\,\ums				&	 &	\\
%$^{125}$Sb				&						& &		&	 &	\\
%$^{190}$Pt				&						& &		&	 &	\\
\hline
\textbf{Holder bulk}	&	Prior (Bq/kg)		& &	\textbf{Holder surfaces}	&	 &	\\
\hline
\ths					&	$<2\times10^{-6}$	& &	$^{210}$Pb\,--\,0.01\,\ums			&	 &	\\
\us 					& $<6.5\times10^{-5}$ 	& &	$^{210}$Pb\,--\,.1\,\ums 			&	 &	\\
\cosn					&$(5\pm1)\times10^{-5}$ & &	$^{210}$Pb\,--\,10\,\ums	    			& 	 &	\\
$^{40}$K				&$(7\pm2)\times10^{-4}$ & &	\ths\,--\,10\,\ums 			&	 &	\\
%$^{54}$Mn
				&						& &	\us\,--\,10\,\ums				&	 &	\\
%$^{57}$Co					&					 &	&		&	 &	\\
\hline
\textbf{Internal Shields}	& Prior (Bq/kg)		& &	\textbf{External Shields}	&	Prior (Bq/kg) &	\\
\hline
\ths					& $<2\times10^{-6}$		& &	\ths				&	 &	\\
\us 					& $<6.5\times10^{-5}$	& &	\us 				&	 &	\\
\cosn 					& $<1.8\times10^{-4}$	& &	\cosn 				& $<4.2\times10^{-5}$ &	\\
$^{40}$K 				&						& &	$^{40}$K			&	 &	\\
%$^{137}$Cs				&						& &						&	 &	\\
\hline
\textbf{Roman Lead}		&	Prior (Bq/kg)		& &\textbf{External Lead}	&	Prior (Bq/kg) &	\\
\hline
\ths					& $<3.3\times10^{-5}$	& &\ths					&	$<2.6\times10^{-4}$ &	\\
\us 					& $<4.5\times10^{-5}$	& &\us					&	$<4.1\times10^{-4}$ &	\\
$^{40}$K				& $<2.3\times10^{-5}$	& &	$^{40}$K			&	$<9\times10^{-3}$ &	\\
%						&						& &	$^{207}$Bi					&	 &	\\
						&						& &	$^{210}$Pb					&	 &	\\
\hline	
\textbf{Other sources}		& Prior (Bq)	 &	&	\textbf{Shields surfaces}	&	 &	\\
\hline
\ths Spot				& $(2.4\pm0.2)\times10^{-4}$& &	50+600mK-$^{210}$Pb			&	 &	\\
$^{40}$K-BottomExtPb	& $16\pm2$					& &	RomanLead-$^{210}$Pb			&	 &	\\
%\hline
%\textbf{Muons}		& (see Sec.~\ref{sec:muons})	 &				&		&	 &	\\
%\hline
\end{tabular}

\end{small}
\end{center}
\label{tab:SourceList} 
\end{table*}

